Scalable Querying of Nested Data

While large-scale distributed data processing platforms have become an attractive target for query processing, these systems are problematic for applications that deal with nested collections. Programmers are forced either to perform non-trivial translations of collection programs or to employ automated flattening procedures, both of which lead to performance problems. These challenges only worsen for nested collections with skewed cardinalities, where both handcrafted rewriting and automated flattening are unable to enforce load balancing across partitions. In this work, we propose a framework that translates a program manipulating nested collections into a set of semantically equivalent shredded queries that can be efficiently evaluated. The framework employs a combination of query compilation techniques, an efficient data representation for nested collections, and automated skew-handling. We provide an extensive experimental evaluation, demonstrating significant improvements provided by the framework in diverse scenarios for nested collection programs.

==> exrun.tex <==
\lstdefinelanguage{NRC}{
  morekeywords={for, in, union, if, then, Sum},%
  sensitive,%
  morecomment=[l]//,%
  morecomment=[s]{/*}{*/},%
  morestring=[b]",%
  morestring=[b]',%
  showstringspaces=false,%
  breaklines=true,%
  mathescape=true,%
  showspaces=false,
  showtabs=false, 
  showstringspaces=false,
  breakatwhitespace=true,
  % xleftmargin=2em,
  % columns=[c]fixed,%
  % basewidth={0.5em, 0.40em},%
  aboveskip=1pt,%\smallskipamount,
  belowskip=1pt,%\negsmallskipamount,
  lineskip=-0.2pt,
%  backgroundcolor=\color{listingbg},
%  basicstyle=\linespread{0.4}\footnotesize\ttfamily,
   % numbers=left,
   % numbersep=5pt,
   % numberstyle=\tiny\ttfamily,
  basicstyle=\ttfamily\color{white!15!black},
  keywordstyle=\ttfamily\bfseries\color{blue!80!black},%
  columns=fullflexible,
%  commentstyle=\commentstyle
  escapeinside={(*@}{@*)}
}[keywords,comments,strings]%

\renewcommand{\bagtype}{\textit{Bag}}
\renewcommand{\stringtype}{\textit{string}}
\newcommand{\datetype}{\textit{date}}
\renewcommand{\doubletype}{\textit{real}}
\renewcommand{\inttype}{\textit{int}}
\renewcommand{\booltype}{\textit{bool}}

\newcommand{\Part}{\texttt{\textup{Part}}}
\newcommand{\Lineitem}{\texttt{Lineitem}}
\renewcommand{\COP}{\texttt{\textup{COP}}}

\renewcommand{\cname}{\texttt{\textup{cname}}}
\renewcommand{\corders}{\texttt{\textup{corders}}}
\renewcommand{\odate}{\texttt{\textup{odate}}}
\renewcommand{\oparts}{\texttt{\textup{oparts}}}
\renewcommand{\pid}{\texttt{\textup{pid}}}
\renewcommand{\lqty}{\texttt{\textup{qty}}}
\renewcommand{\pname}{\texttt{\textup{pname}}}
\renewcommand{\total}{\texttt{\textup{total}}}
\newcommand{\punto}{$\hspace*{\fill}\Box$}

\begin{example} \label{ex:run}
Consider a variant of the TPC-H database containing a flat relation $\Part$ with information about parts and a nested relation $\COP$ with information about customers, their orders, and the parts purchased in the orders.
The relation $\COP$ stores customer names, order dates, and part IDs and purchased quantities per order. The type of $\COP$ is: 
\begin{align*}
\bagtype\,(\<\, & \cname:\stringtype,\, \corders:\bagtype\,(\<\, \odate: \datetype, \\[-2pt]
& \hspace{1.8cm}\oparts: \bagtype\,(\<\, \pid: \inttype,\, \lqty: \doubletype \,\>) \,\>) \,\>).
\end{align*}

Consider a query that computes for each customer and for each their order, the total amount spent grouped by the part name. 
This query requires joining $\COP$ with $\Part$ on $\pid$ to get the name and price of each part and then aggregating per part name. We can express this query in $\nrc$ as:

{\em
\vspace{3pt}
\begin{lstlisting}[language=NRC, ]
for $\texttt{cop}$ in $\texttt{COP}$ union
  $\{\<\, \texttt{cname} \ateq \texttt{cop}.\texttt{cname},$ $\texttt{corders} \ateq$ 
        for $\texttt{co}$ in $\texttt{cop}.\texttt{corders}$ union
          $\{\<\, \texttt{odate} \ateq \texttt{co}.\texttt{odate},$ $\texttt{oparts} \ateq$ Sum$_{\hspace{0.3mm}\texttt{pname}}^{\hspace{0.3mm}\texttt{total}}($
                for $\texttt{op}$ in $\texttt{co.oparts}$ union
                  for $\texttt{p}$ in $\texttt{Part}$ union
                    if $\texttt{op}.\texttt{pid} == \texttt{p}.\texttt{pid}$ then
                      $\{\<\, \texttt{pname} \ateq \texttt{p}.\texttt{pname},$
                        $\,\texttt{total} \ateq \texttt{op}.\texttt{qty} * \texttt{p}.\texttt{price} \,\>\})\,\>\}\,\>\}$
\end{lstlisting}
}

The query navigates to the bags $\oparts$ in $\COP$, then joins each of them with $\Part$, and computes group-by aggregates using the 
$\textup{\texttt{Sum}}$ construct: for each distinct part name, it sums up the total amount spent.
The output type of this query is:
\begin{align*}
&\bagtype\,(\<\, \cname:\stringtype,\, \corders:\bagtype\,(\<\, \odate: \datetype, \\[-2pt]
& \hspace{1.4cm} \oparts: \bagtype\,(\<\, \pname: \stringtype,\, \total: \doubletype \,\>)\, \>)\, \>).%\phantom{\quad\textrm{$\Box$}}
\end{align*}
% This query performs nested joins among the three levels of bags.
% We perform aggregation on the third level by using the $\texttt{Sum}$ construct: for each part (grouped using the attribute \pname), it computes the summation of the total amount spent (using the attribute \total).
% \punto
\end{example}



==> macrosart.tex <==
\renewcommand{\Join}{\bowtie}
\lstdefinelanguage{NRC}{
  morekeywords={for, in, union, if, then, else, match, let},%
  sensitive,%
  morecomment=[l]//,%
  morecomment=[s]{/*}{*/},%
  morestring=[b]",%
  morestring=[b]',%
  showstringspaces=false,%
  breaklines=true,%
  mathescape=true,%
  showspaces=false,
  showtabs=false, 
  showstringspaces=false,
  breakatwhitespace=true,
  % xleftmargin=2em,
  % columns=[c]fixed,%
  % basewidth={0.5em, 0.40em},%
  aboveskip=1pt,%\smallskipamount,
  belowskip=1pt,%\negsmallskipamount,
  lineskip=-0.2pt,
%  backgroundcolor=\color{listingbg},
%  basicstyle=\linespread{0.4}\footnotesize\ttfamily,
   % numbers=left,
   % numbersep=5pt,
   % numberstyle=\tiny\ttfamily,
  basicstyle=\ttfamily\color{white!15!black},
  keywordstyle=\ttfamily\bfseries\color{blue!80!black},%
  columns=fullflexible,
%  commentstyle=\commentstyle
  escapeinside={(*@}{@*)}
}[keywords,comments,strings]%

\lstdefinelanguage{Scala}%
{morekeywords={abstract,%
  case,catch,char,class,%
  def,else,extends,final,finally,for,%
  if,import,implicit,%
  match,module,%
  new,null,%
  object,override,%
  package,private,protected,public,%
  for,public,return,super,%
  this,throw,trait,try,type,%
  val,var,%
  with,while,%
  yield%
  },%
  sensitive,%
  morecomment=[l]//,%
  morecomment=[s]{/*}{*/},%
  morestring=[b]",%
  morestring=[b]',%
  showstringspaces=false,%
    breaklines=true,%
  mathescape=true,%
  showspaces=false,
  showtabs=false,
  showstringspaces=false,
  breakatwhitespace=true,
  xleftmargin=2em,
%  columns=[c]fixed,%
%  basewidth={0.5em, 0.40em},%
  aboveskip=1pt,%\smallskipamount,
  belowskip=1pt,%\negsmallskipamount,
  lineskip=-0.2pt,
%  basewidth={0.54em, 0.4em},%
%  backgroundcolor=\color{listingbg},
%  basicstyle=\linespread{0.4}\footnotesize\ttfamily,
%  keywordstyle=\keywordstyle,
   % numbers=left,
   % numbersep=5pt,
   % numberstyle=\tiny\ttfamily,
   basicstyle=\ttfamily,
  % keywordstyle=\ttfamily\bfseries,%
  keywordstyle=\ttfamily\color{blue!80!black},
  columns=fullflexible,
%  commentstyle=\commentstyle
  %xleftmargin=1ex
  % escapeinside={(*@}{@*)}
}[keywords,comments,strings]%

\newcounter{magicrownumbers}
\newcommand\rownumber{\stepcounter{magicrownumbers}\arabic{magicrownumbers}}
\newcommand{\linenumber}{\makebox[2ex][r]{$\scriptscriptstyle\rownumber\;\;$}}

% General
\newcommand{\myeat}[1]{}
\newcommand{\punto}{$\hspace*{\fill}\Box$}
\newcommand{\NULL}{\texttt{NULL}}
\newcommand{\tab}{\;\;\;}
\newcommand\mydots{\makebox[1em][c]{.\hfil.\hfil.}}

% Comments
\newcommand{\michael}[1]{{\bf Michael: #1}}
%\newcommand{\michael}[1]{}
%\newcommand{\amir}[1]{{\bf \color{blue} Amir: #1}}
%\newcommand{\jac}[1]{{\bf \color{violet} Jaclyn: #1}}
\newcommand{\milos}[1]{{\bf \color{red} Milos: #1}}

% Types
\newcommand{\bagtype}{\textit{Bag}\hspace{0.5mm}}
\newcommand{\labeltype}{\textit{Label}\xspace}
\newcommand{\stringtype}{\textit{string}}
\newcommand{\datetype}{\textit{date}}
\newcommand{\doubletype}{\textit{real}}
\newcommand{\inttype}{\textit{int}}
\newcommand{\booltype}{\textit{bool}}

% Running example
\newcommand{\Part}{\texttt{\textup{Part}}\xspace}
\newcommand{\Lineitem}{\texttt{Lineitem}\xspace}
\newcommand{\COP}{\texttt{\textup{COP}}\xspace}
\newcommand{\cid}{\texttt{\textup{cid}}\xspace}
\newcommand{\cname}{\texttt{\textup{cname}}\xspace}
\newcommand{\corders}{\texttt{\textup{corders}}\xspace}
\newcommand{\odate}{\texttt{\textup{odate}}\xspace}
\newcommand{\oparts}{\texttt{\textup{oparts}}\xspace}
\newcommand{\pid}{\texttt{\textup{pid}}\xspace}
\newcommand{\pname}{\texttt{\textup{pname}}\xspace}
\newcommand{\pprice}{\texttt{\textup{price}}\xspace}
\newcommand{\lqty}{\texttt{\textup{qty}}\xspace}
\newcommand{\total}{\texttt{\textup{total}}\xspace}
\newcommand{\pkey}{\texttt{\textup{id}}\xspace}
\newcommand{\sumBy}{\texttt{\textup{sumBy}}}

% TPCH Benchmark
\newcommand{\Order}{\texttt{Order}\xspace}
\newcommand{\Customer}{\texttt{Customer}\xspace}
\newcommand{\Region}{\texttt{Region}\xspace}
\newcommand{\rid}{\texttt{\textup{rid}}\xspace}
\newcommand{\rname}{\texttt{\textup{rname}}\xspace}
\newcommand{\rnations}{\texttt{\textup{rnations}}\xspace}
\newcommand{\Nation}{\texttt{Nation}\xspace}
\newcommand{\nid}{\texttt{\textup{nid}}\xspace}
\newcommand{\nname}{\texttt{\textup{nname}}\xspace}
\newcommand{\ncusts}{\texttt{\textup{ncusts}}\xspace}
\newcommand{\oid}{\texttt{\textup{oid}}\xspace}
\newcommand{\RNCOP}{\texttt{\textup{RNCOP}}\xspace}
\newcommand{\cogroup}{\texttt{\kw{COGROUP}}\xspace}

% Bio Benchmark
\newcommand{\Occur}{\texttt{Occurrences}\xspace}
\newcommand{\OccurGroup}{\texttt{OccurGrouped}\xspace}
\newcommand{\OccurJoin}{\texttt{OccurCNVJoin}\xspace}
\newcommand{\OccurAgg}{\texttt{OccurCNVAgg}\xspace}
\newcommand{\CopyNum}{\texttt{CopyNumber}\xspace}
\newcommand{\Pathway}{\texttt{Pathway}\xspace}
\newcommand{\GeneExpr}{\texttt{GeneExpression}\xspace}
\newcommand{\Biospec}{\texttt{Samples}\xspace}
\newcommand{\SOImpact}{\texttt{SOImpact}\xspace}
\newcommand{\Network}{\texttt{Network}\xspace}
\newcommand{\MNetwork}{\texttt{MappedNetwork}\xspace}
\newcommand{\FNetwork}{\texttt{FNetwork}\xspace}
\newcommand{\SNetwork}{\texttt{SampleNetwork}\xspace}
\newcommand{\Biomart}{\texttt{Biomart}\xspace}
\newcommand{\Hybrid}{\texttt{HybridMatrix}\xspace}
\newcommand{\Effect}{\texttt{EffectMatrix}\xspace}
\newcommand{\Connect}{\texttt{ConnectMatrix}\xspace}
\newcommand{\Connects}{\texttt{Connectivity}\xspace}
\newcommand{\aid}{\texttt{\textup{aid}}\xspace}
\newcommand{\aliquot}{\texttt{\textup{aliquot}}\xspace}
\newcommand{\sample}{\texttt{\textup{sample}}\xspace}
\newcommand{\gid}{\texttt{\textup{gid}}\xspace}
\newcommand{\gene}{\texttt{\textup{gene}}\xspace}
\newcommand{\protein}{\texttt{\textup{protein}}\xspace}
\newcommand{\impact}{\texttt{\textup{impact}}\xspace}
\newcommand{\conseq}{\texttt{\textup{conseq}}\xspace}
\newcommand{\cnum}{\texttt{\textup{cnum}}\xspace}
\newcommand{\trans}{\texttt{\textup{transcripts}}\xspace}
\newcommand{\cands}{\texttt{\textup{candidates}}\xspace}
\newcommand{\nodes}{\texttt{\textup{nodes}}\xspace}
\newcommand{\conseqs}{\texttt{\textup{consequences}}\xspace}
\newcommand{\hyscores}{\texttt{\textup{scores}}\xspace}
\newcommand{\hscore}{\texttt{\textup{score}}\xspace}
\newcommand{\sift}{\texttt{\textup{sift}}\xspace}
\newcommand{\siftpred}{\texttt{\textup{siftpredict}}\xspace}
\newcommand{\poly}{\texttt{\textup{poly}}\xspace}
\newcommand{\polypred}{\texttt{\textup{polypredict}}\xspace}
\newcommand{\proj}{\texttt{\textup{project}}\xspace}
\newcommand{\nodep}{\texttt{\textup{nodeProtein}}\xspace}
\newcommand{\edges}{\texttt{\textup{edges}}\xspace}
\newcommand{\edgep}{\texttt{\textup{edgeProtein}}\xspace}
\newcommand{\score}{\texttt{\textup{score}}\xspace}
\newcommand{\genes}{\texttt{\textup{genes}}\xspace}
\newcommand{\mutations}{\texttt{\textup{mutations}}\xspace}
\newcommand{\dist}{\texttt{\textup{distance}}\xspace}
\newcommand{\case}{\texttt{\textup{case}}\xspace}
\newcommand{\contig}{\texttt{\textup{contig}}\xspace}
\newcommand{\mstart}{\texttt{\textup{start}}\xspace}
\newcommand{\mend}{\texttt{\textup{end}}\xspace}
\newcommand{\mref}{\texttt{\textup{reference}}\xspace}
\newcommand{\alt}{\texttt{\textup{alternate}}\xspace}
\newcommand{\mutid}{\texttt{\textup{mutationId}}\xspace}
\newcommand{\uid}{\texttt{\textup{uid}}\xspace}
\newcommand{\gibbs}{\texttt{\textup{gibbs}}\xspace}
\newcommand{\extern}{\texttt{\textup{external}}\xspace}
\newcommand{\interm}{\texttt{\textup{E}}\xspace}
\newcommand{\fpkm}{\texttt{\textup{fpkm}}\xspace}
\newcommand{\pathway}{\texttt{\textup{pathway}}\xspace}
\newcommand{\pathways}{\texttt{\textup{pathways}}\xspace}
\newcommand{\burden}{\texttt{\textup{burden}}\xspace}


% NRC
\newcommand{\nrcagg}{\kw{NRC}}
\newcommand{\nrcaggshr}{\nrcagg^{Lbl+\lambda}}
\newcommand{\nrcaggshrmat}{\nrcagg^{Lbl}}

\newcommand{\kwd}[1]{\texttt{\textup{#1}}\xspace}
\newcommand{\idfor}{\kwd{for}}
\newcommand{\idin}{\kwd{in}}
\newcommand{\idunion}{\kwd{union}}
\newcommand{\idif}{\kwd{if}}
\newcommand{\idthen}{\kwd{then}}
\newcommand{\idelse}{\kwd{else}}
\newcommand{\idlet}{\kwd{let}}
\newcommand{\idmatch}{\kwd{match}}

\newcommand{\ckwd}[1]{\kwd{\color{blue!80!black} #1}}
\newcommand{\cidfor}{\ckwd{\idfor}}
\newcommand{\cidin}{\ckwd{\idin}}
\newcommand{\cidunion}{\ckwd{\idunion}}
\newcommand{\cidif}{\ckwd{\idif}}
\newcommand{\cidthen}{\ckwd{\idthen}}
\newcommand{\cidelse}{\ckwd{\idelse}}
\newcommand{\cidlet}{\ckwd{\idlet}}
\newcommand{\cidmatch}{\ckwd{\idmatch}}

\newcommand{\getkw}{\kwd{get}}
\newcommand{\dedup}{\kwd{dedup}}
\newcommand{\groupby}{\kwd{groupBy}}
\newcommand{\sumby}{\kwd{sumBy}}
\newcommand{\lookup}{\kwd{Lookup}}
\newcommand{\dicttreeunion}{\kwd{DictTreeUnion}}
\newcommand{\newlabelof}{\kwd{NewLabel}}
\newcommand{\matlookup}{\kwd{MatLookup}}
\newcommand{\flatc}{\textup{F}}
\newcommand{\dictc}{\textup{D}}
\newcommand{\shredf}[1]{\mathcal{F}(#1)}
\newcommand{\shredd}[1]{\mathcal{D}(#1)}
\newcommand{\FUN}{\kwd{fun}}
\newcommand{\CHILD}{\kwd{child}}
\newcommand{\dictunion}{\kwd{DictUnion}}

\newcommand{\groupatt}{\kwd{group}}
\newcommand{\labelatt}{\kwd{label}}
\newcommand{\valueatt}{\kwd{value}}

\newcommand{\olabelatt}{\kwd{olabel}}
\newcommand{\clabelatt}{\kwd{clabel}}
\newcommand{\nlabelatt}{\kwd{nlabel}}
\newcommand{\rlabelatt}{\kwd{rlabel}}

\newcommand{\topbag}{\kw{TopBag}}
\newcommand{\labeldomain}{\kw{LabDomain}}

% Algebra
\newcommand{\bagunion}{\uplus}




\newcommand{\vshred}{\kw{vshred}}
\newcommand{\vunshred}{\kw{vunshred}}
\newcommand{\labelcode}{\kw{idgen}}

\newcommand{\matdict}{\kw{MatDict}}
\newcommand{\shredalg}{\kw{ShredQ}}
\newcommand{\sysname}{\kw{BINDS}}
\newcommand{\abinterp}{\kw{AbInterp}}
\newcommand{\langeq}{==}
\newcommand{\join}{\bowtie}
%\newtheorem{example}{Example}
%\newtheorem{theorem}{Theorem}
% \newcommand{\lookup}{\kw{Lookup}}
% \newcommand{\idif}{\kw{If}}
% \newcommand{\idthen}{\kw{Then}}
% \newcommand{\idelse}{\kw{Else}}
% \newcommand{\groupby}{\kw{GroupBy}}
% \newcommand{\sumkw}{\kw{Sum}}
% \newcommand{\getkw}{\kw{Get}}
% \newcommand{\groupbyplus}[4]{\sumkw_{#1}^{#2}(#3, #4)}
% \newcommand{\coloneq}{~:=~}
\newcommand{\ateq}{:=}
\newcommand{\leteq}{:=}
\newcommand{\assigneq}{\Leftarrow}
\newcommand{\sng}[1]{\{ #1 \}}

\newcommand{\linearize}{\kw{Linearize}\xspace}
\newcommand{\materialize}{\kw{Materialize}\xspace}
\newcommand{\translate}{\kw{Translate}\xspace}
\newcommand{\bagtomatdict}{\texttt{BagToDict}\xspace}
\newcommand{\agg}{\kw{AGG}\xspace}
\newcommand{\heavykeys}{\texttt{heavyKeys}\xspace}

% \newcommand{\patientinfo}{\kw{pinfo}}
% \newcommand{\genotypes}{\kw{gtypes}}
% \newcommand{\clinical}{\kw{Clinical}}
% \newcommand{\sample}{\kw{sample}}
% \newcommand{\samples}{\kw{samples}}
% \newcommand{\keys}{\kw{keys}}

% \newcommand{\wmcc}{\kw{WMCC}}
% \newcommand{\setcomp}{\kw{SetComp}}
% \newcommand{\countcomp}{\kw{CountComp}}
% \newcommand{\generatedby}{\leftarrow}
% \newcommand{\weightby}{\kw{WeightBy}}
% \newcommand{\bagcomp}{\kw{BagComp}}
% \newcommand{\bagcomprehension}{\bagcomp}
% \newcommand{\idfor}{\kw{For}}
% \newcommand{\idlet}{\kw{Let}}
% \newcommand{\idunion}{\kw{Union}}
% \newcommand{\gensingletoncon}{\kw{WSC}}
% \newcommand{\idin}{\kw{In}}
% \newcommand{\dedup}{\kw{DeDup}}
\newcommand{\oplang}{\kw{OPL}}
\newcommand{\totalmult}{\kw{TotalMult}}
\newcommand{\topout}{\kw{OutTopSubq}}
\newtheorem{proposition}{Proposition}
\newcommand{\renaming}{\kw{Relabeling}}
\newcommand{\relabeling}{\renaming}
\newcommand{\mapunion}{\kw{MapUnion}}
% \newcommand{\dictunion}{\kw{DictUnion}}
\newcommand{\topdict}{\kw{TopDict}}
\newcommand{\fulldict}{\dict}
\newcommand{\inputlabels}{\kw{InputLabels}}
\newcommand{\nrcplus}{NRC^+}
\newcommand{\nrc}{\kw{NRC}}
\newcommand{\freevars}{\kw{FreeVar}}
\newcommand{\transformbag}{\kw{TransformQueryBag}}
\newcommand{\transformtuple}{\kw{TransformQueryTuple}}
\newcommand{\transformtupleelement}{\kw{TransformQueryTupleElement}}
\newcommand{\pretransformbag}{\kw{TransformQueryBagAux}}
\newcommand{\outputlabels}{\kw{OutputLabels}}
\newcommand{\inputdict}{\kw{InputDict}}
\newcommand{\extractfromlabel}{\kw{Extrctval}}
\newcommand{\extracttag}{\kw{Extrcttag}}
\newcommand{\extract}{\extractfromlabel}
\newcommand{\extractfromlabelall}{\kw{ExtractFromLabelAll}}
\newcommand{\simplenrc}{\kw{SimpleNRC}}
\newcommand{\simplenrclet}{\kw{SimpleNRC}^{\kw{Let}}}
\newcommand{\nextmaximal}{\kw{NextMaximal}}
\newcommand{\mult}{\kw{Mult}}
\newcommand{\maximalsubexpressions}{\kw{MaxSub}}
\newcommand{\parent}{\kw{Parent}}
\newcommand{\typeof}{\kw{TypeOf}}



% \newcommand{\labeltype}{\kw{Label}}
% \newcommand{\bagtype}{\kw{Bag}}
% \newcommand{\stringtype}{\kw{Str}}
% \newcommand{\doubletype}{\kw{Dbl}}
% \newcommand{\inttype}{\kw{Int}}
% \newcommand{\booltype}{\kw{Bool}}
% \newcommand{\settype}{\kw{SetType}}
% \newcommand{\attributedomain}{\kw{AttributeDomain}}
% \newcommand{\tupletype}{\kw{TupleType}}
% \newcommand{\bagof}{\kw{BagOf}}
% \newcommand{\scalartype}{\kw{Scalar}}
% \newcommand{\idmatch}{\kw{Match}}
% \newcommand{\singleton}{\kw{sng}}


% \newcommand{\COP}{\kw{COP}}
% \newcommand{\Parts}{\kw{Part}}


% \newcommand{\corders}{\kw{corders}}
% \newcommand{\pname}{\kw{pname}}
% \newcommand{\pid}{\kw{pid}}
% \newcommand{\partid}{\pid}
% \newcommand{\oparts}{\kw{oparts}}
% \newcommand{\cname}{\kw{cname}}
% \newcommand{\odate}{\kw{odate}}
% \newcommand{\lqty}{\kw{lqty}}
% \newcommand{\pretailprice}{\kw{price}}
% \newcommand{\total}{\kw{total}}

% \newcommand{\topbag}{\kw{TopBag}}
% \newcommand{\valueatt}{\kw{value}}
% \newcommand{\labelatt}{\kw{label}}
% \newcommand{\keyatt}{\kw{key}}

\newcommand{\variants}{\kw{Variants}}
\newcommand{\gensingleton}{\kw{WeightedSing}}
\newcommand{\flatten}{\kw{Flatten}}
% \newcommand{\newlabelof}{\kw{New}}
\newcommand{\indextype}{\kw{IndexType}}
\newcommand{\indicesof}{\kw{IndicesOf}}
\newcommand{\evalexpr}[2]{{\llbracket #1\rrbracket}_{#2}}
\newcommand{\shredobj}{\kw{Shredded}}
\newcommand{\shreddedvars}{\kw{ShreddedVars}}
\newcommand{\emptydict}{\langle \rangle}
\newcommand{\outcome}[3][]{\ensuremath{\llbracket#2\ifstrempty{#1}{}{\mid#1}\rrbracket_{#3}}}
\newcommand{\interpret}[2]{\outcome{#1}{#2}}
\newcommand{\IdFor}{\kw{For}}
\newcommand{\emptytype}{()}
\newcommand{\IdUnion}{\kw{Union}}
\newcommand{\IdIn}{\kw{In}}
\newcommand{\queryunion}{\uplus}
\newcommand{\tuple}[1]{{\langle#1\rangle}}
\newcommand{\pred}{pred}
\newcommand{\emptybag}{\{\}_{\bagtype(T)}}
\newcommand{\emptybagq}{\emptyset_{\bagtype(F)}}
\newcommand{\emptybaggen}[1]{\emptyset_{\bagtype(#1)}}
\newcommand{\emptysetq}{\emptyset_{\settype(T)}}
\def\lBrack{\lbrack\!\lbrack}
\def\rBrack{\rbrack\!\rbrack}
\newcommand{\Bracks}[1]{\lBrack#1\rBrack}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}



\newcommand{\datalogarrow}{ :=}
\newcommand{\aschema}{\mathcal{S}}
\newcommand{\powerset}[1]{\mathcal{P}(#1)}
\newcommand{\LFPP}[3]{\LFP_{#1,#2}^{#3}}
\newcommand{\LFPA}[2]{\LFP_{#1,#2}}
\newcommand{\GFPA}[2]{\GFP_{#1,#2}}
\newcommand{\nf}{\text{strict normal form}\xspace}
\newcommand{\logic}[1]{\textup{\small #1}\xspace}
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\A}{\mathbb{A}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Ninf}{\mathbb{N_\infty}}
\newcommand{\fA}{\mathfrak{A}}
\newcommand{\fB}{\mathfrak{B}}
\newcommand{\fU}{\mathfrak{U}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\set}[1]{\left\{{#1}\right\}}
\newcommand{\sset}[1]{\{{#1}\}}
\newcommand{\size}[1]{\lvert #1 \rvert}
\newcommand{\width}[1]{\operatorname{width}( #1 )}
\newcommand{\restrict}[2]{ #1\restriction_{#2} }
\let\Lslash\L
\renewcommand{\L}{\mathrm{L}}
\newcommand{\R}{\mathrm{R}}
\newcommand{\interpolant}[1]{\theta_{#1}}
\newcommand{\free}[1]{\operatorname{free}(#1)}
\newcommand{\dom}[1]{\operatorname{dom}(#1)}
\newcommand{\gn}{\textup{GN}\xspace}
\newcommand{\gnfo}{\logic{GNF}}
\newcommand{\gso}{\logic{GSO}}
\newcommand{\mso}{\logic{MSO}}
\newcommand{\gnf}{\gnfo}
\newcommand{\gf}{\logic{GF}}
\newcommand{\lfp}{\logic{LFP}}
\newcommand{\unfo}{\logic{UNF}}
\newcommand{\fo}{\logic{FO}}
\newcommand{\unf}{\unfo}
\newcommand{\Lmu}{\textup{L}_{\mu}}
\newcommand{\gnfpup}{\logic{GNFP-UP}}
\newcommand{\unfpup}{\logic{UNFP-UP}}
\newcommand{\gnfpplus}{\gnfpup}
\newcommand{\unfpplus}{\unfpup}
\newcommand{\GFP}{\operatorname{\bf gfp}}
\newcommand{\gfp}{\logic{GFP}}
\newcommand{\LFP}{\operatorname{\bf lfp}}
\newcommand{\unravel}[1]{\cT(#1)}
\newcommand{\gnfp}{\logic{GNFP}}
\newcommand{\unfp}{\logic{UNFP}}
\newcommand{\unfpk}{\unfp^k}
\newcommand{\gnfk}{\gnf^k}
\newcommand{\unfk}{\unf^k}
\newcommand{\lfpl}{\logic{LFP}}
\newcommand{\complexity}[1]{\textsc{#1}}
\newcommand\ptime{\complexity{PTime}\xspace}
\newcommand\exptime{\complexity{ExpTime}\xspace}
\newcommand\nexptime{\complexity{NExpTime}\xspace}
\newcommand\twoexptime{\complexity{2-ExpTime}\xspace}
\newcommand{\twoexp}{\twoexptime}
\newcommand\np{\complexity{NP}\xspace}
\newcommand\conp{\complexity{co-NP}\xspace}
\newcommand{\dmodality}[1]{\langle #1 \rangle}
\newcommand{\bmodality}[1]{[ #1 ]}
\newcommand{\valuation}{\ell}
\newcommand{\codom}[1]{\operatorname{rng}(#1)}
\newcommand{\decode}[1]{\mathfrak{D}(#1)}
\newcommand{\tree}{\cT}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\gnfpk}{\text{$\gnfp^k$}\xspace}
\renewcommand{\varphi}{\phi}
\newcommand{\kw}[1]{\textsc{#1}}
\newcommand{\atypesig}[3]{\kw{AT}_{#2,#3}(#1)}
\newcommand{\ExactLabel}[1]{\kw{ExactLabel}(#1)}
\newcommand{\GNLabel}[1]{\kw{GNLabel}(#1)}
\newcommand{\sigmag}{\sigma_g}
\newcommand{\sigmaprimeg}{\sigma'_g}
\newcommand{\gnl}{\gn^{l}}
\newcommand{\sigk}{\tilde{\sigma}_k}
\newcommand{\gnkinvar}{\logic{GN}^k}
\newcommand{\sgnkinvar}{\logic{BGN}^k}
\newcommand{\sunkinvar}{\logic{BUN}^k}
\newcommand{\gnlinvar}{\logic{GN}^l}
\newcommand{\gnninvar}{\logic{GN}^n}
\newcommand{\gnminvar}{\logic{GN}^m}
\newcommand{\ginvar}{\logic{G}}
\newcommand{\bunravelk}[2]{\cU_{\textup{BGN}^k[#2]}( #1 )}
\newcommand{\unravelk}[2]{\cU_{\textup{GN}^k[#2]}( #1 )}
\newcommand{\unravelm}[2]{\cU_{\textup{GN}^m[#2]}( #1 )}
\newcommand{\unravell}[2]{\cU_{\textup{GN}^l[#2]}( #1 )}
\newcommand{\sunravelk}[2]{\cU^{\textup{plump}}_{\textup{BGN}^k[#2]}( #1 )}
\newcommand{\gunravel}[2]{\cU_{\textup{G}[#2]}( #1 )}
\newcommand{\sigcode}[2]{\Sigma^{\text{code}}_{#1,#2}}
\newcommand{\dloglite}{\logic{DATALOG-LITE}}
\newcommand{\dlog}{\logic{DATALOG}}
\newcommand{\unravellingcode}{\cU_{\logictarget}(\fB)}
\newcommand{\lemmafwd}{\hyperref[lemma:forward-gso]{Lemma~Fwd}\xspace}
\newcommand{\lemmagfpbwd}[1]{\hyperref[lemma:backwards-gfp]{#1}\xspace}
\newcommand{\lemmagnfpbwd}[1]{\hyperref[lemma:backwards-gnfp]{#1}\xspace}
\newcommand{\logictarget}{\cL_1}
\newcommand{\sigtarget}{\sigma'}
\newcommand{\sigoriginal}{\sigma}
\newcommand{\Bekic}{Beki\v{c}\xspace}
\newcommand{\convertnf}[1]{\operatorname{convert}(#1)}
\newcommand{\indices}[1]{\textup{names}(#1)}
\newcommand{\dup}{\uparrow}
\newcommand{\dstay}{0}
\newcommand{\ddown}{\downarrow}
\newcommand{\Pri}{\mathrm{Pri}}
\newcommand{\Dir}{\mathrm{Dir}}
\newcommand{\gameonstart}[3]{\cG(#1, #2, #3)}
\newcommand{\gameon}[2]{\cG(#1, #2)}
\newcommand{\Sigmap}{\Sigma_p}
\newcommand{\Sigmaa}{\Sigma_a}
\newcommand{\QE}{Q_{E}}
\newcommand{\QA}{Q_{A}}
\newcommand{\simgn}[1]{\sim_{#1}}
\newcommand{\subsetgn}[1]{\subseteq_{#1}}
\newcommand{\remove}[2]{\text{remove}_{#2}(#1)}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\namesk}{U_k}
\newcommand{\atype}[2]{\kw{AT}_{#2}(#1)}
\newcommand{\propsguardedneg}[1]{\kw{GNProps}(#1)}
\newcommand{\propsneg}[1]{\kw{NProps}(#1)}
\newcommand{\bagextend}[1]{\kw{BagLabels}(#1)}
\newcommand{\GuardedLabels}{\kw{GLabels}}
\newcommand{\GuardedLabelsNeighbor}[2]{\kw{GLabels}(#1,#2)}
\newcommand{\IntNodeLabels}{\kw{InterfaceLabels}}
\newcommand{\BagNodeLabels}{\kw{BagLabels}}
\newcommand{\EdgeLabels}{\kw{Edges}}
\newcommand{\EdgeLabelsRestrict}[1]{\kw{Edges}(#1)}
\newcommand{\NodeLabels}{\kw{NodeLabels}}
\newcommand{\tforward}[1]{ {#1}^{\rightarrow} }
\newcommand{\tbackward}[1]{ {#1}^{\leftarrow} }
\newcommand{\struct}[1]{\mathfrak{D}(#1)}
\newcommand{\readymode}{\text{select}}
\newcommand{\waitmode}{\text{move}}
\newcommand{\views}{\kw{Views}}
\newcommand{\view}{I}
\newcommand{\dneighbor}{\updownarrow}
\newcommand{\strategy}{\zeta}
\newcommand{\correct}[1]{\textup{correct}(#1)}
\newcommand{\correctr}[1]{\textup{correct}_{r}(#1)}
\newcommand{\Fpart}[1]{\textup{match}(#1)}
\newcommand{\id}{\textup{id}}
\newcommand{\consistencyform}{\phi_{\textup{consistent}}}
\newcommand{\elem}[1]{\operatorname{elem}(#1)}
\newcommand{\guardg}[2]{\operatorname{guard}^{\sigmag}_{#1}(#2)}
\newcommand{\Guarded}[1]{\kw{Gdd}(#1)}
\newcommand{\GuardedDom}[1]{\guardedg_{\dom{#1}}} 
\newcommand{\GuardedRng}[1]{\guardedg_{\codom{#1}}} 
\newcommand{\GuardDom}[2]{\operatorname{guard-dom}(#1,#2)} 
\newcommand{\GuardRng}[2]{\operatorname{guard-rng}(#1,#2)}
\newcommand{\phiL}{\phi_{\L}}
\newcommand{\phiR}{\phi_{\R}}
\newcommand{\cform}[2]{\text{consistent}_{#1,#2}}
\newcommand{\sigR}{\sigma_{\R}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\gnnf}{\text{\textup{GN}-normal form}\xspace}
\newcommand{\myparagraph}[1]{{\bf #1.}}
\newcommand{\true}{\kw{True}}
\newcommand{\false}{\kw{False}}

\newcommand{\mattranstwo}[2]{\mathcal{M}\lBrack#1\rBrack_{#2}}
\newcommand{\mattransbasic}[2]{\mathcal{M}\lBrack#1\rBrack_{#2}}
\newcommand{\mattrans}[3]{\mattranstwo{#1}{#2,#3}}

%experiments
\newcommand{\Flat}{\kw{Flat}\xspace}
\newcommand{\Fplus}{$\kw{Flat}^+$\xspace}
%\newcommand{\Fpplus}{$\Flat^{++}$\ }
%\newcommand{\Fpplus}{\kw{Flat}\xspace}
\newcommand{\Fpplus}{\kw{Std} \xspace}

%biostuff
\newcommand{\bioendtoend}{\kw{E2E}}
\newcommand{\Stepi}{$\kw{Step}_1$\xspace}
\newcommand{\Stepii}{$\kw{Step}_2$\xspace}
\newcommand{\Stepiii}{$\kw{Step}_3$\xspace}
\newcommand{\Stepiv}{$\kw{Step}_4$\xspace}
\newcommand{\Stepv}{$\kw{Step}_5$\xspace}
\newcommand{\Ci}{$\kw{C}_1$\xspace}
\newcommand{\Cii}{$\kw{C}_2$\xspace}
\newcommand{\Ciii}{$\kw{C}_3$\xspace}
\newcommand{\OccurFull}{$\kw{BN}_2$\xspace}
%\newcommand{\OccurSmall}{$\kw{BN}_2$\xspace}
\newcommand{\CNVFull}{$\kw{BF}_2$\xspace}
%\newcommand{\CNVSmall}{$\kw{DF}_3^{Small}$\xspace}
\newcommand{\ExprFull}{$\kw{BF}_1$\xspace}
%\newcommand{\ExprSmall}{$\kw{DF}_1^{Small}$\xspace}
\newcommand{\NetworkFull}{$\kw{BN}_1$\xspace}
\newcommand{\SeqOnto}{$\kw{BF}_3$\xspace}


\newcommand{\superunshred}{\kw{U}}
%michael: can change this above back to unshred
\newcommand{\Shred}{\kw{Shred}\xspace}
\newcommand{\Unshred}{\kw{Unshred}\xspace}
\newcommand{\Shrdom}{$\Shred^{\kw{Dom}}$\xspace}
\newcommand{\Fskew}{$\Flat_{\kw{skew}}$\xspace}
\newcommand{\Sskew}{$\Shred_{\kw{skew}}$\xspace}
\newcommand{\Uskew}{$\Shred_{\kw{skew}}^{+ \superunshred}$\xspace}
\newcommand{\Sdskew}{$\Shred^{\kw{Dom}}_{\kw{skew}}$\xspace}


\DeclareRobustCommand{\ojoin}{\rule[0.10ex]{.3em}{.4pt}\llap{\rule[1.40ex]{.3em}{.4pt}}}
\newcommand{\leftouterjoin}{\mathrel{\ojoin\mkern-6.5mu\Join}}
\newcommand{\rightouterjoin}{\mathrel{\Join\mkern-6.5mu\ojoin}}
\DeclareRobustCommand{\ounnest}{\rule[2.0ex]{.3em}{.4pt}\llap{\rule[1.0ex]{.3em}{.4pt}}}
% \newcommand{\outerunnest}{\mathrel{\ounnest\mkern-1.6mu\mu}}
\newcommand\textequal{%
 \rule[.3ex]{3pt}{0.4pt}\llap{\rule[.7ex]{3pt}{0.4pt}}}
\newcommand{\outerunnest}{\mathrel{\textequal\!\mu}}

\newtheorem{example}{Example}

